Unifying Semantic Foundations for Automated Verification Tools in Isabelle/UTP

The growing complexity and diversity of models used in the engineering of dependable systems implies that a variety of formal methods, across differing abstractions, paradigms, and presentations, must be integrated. Such an integration relies on unified semantic foundations for the various notations, and co-ordination of a variety of automated verification tools. The contribution of this paper is Isabelle/UTP, an implementation of Hoare and He's Unifying Theories of Programming, a framework for unification of formal semantics. Isabelle/UTP permits the mechanisation of computational theories for diverse paradigms, and their use in constructing formalised semantic models. These can be further applied in the development of verification tools, harnessing Isabelle's proof automation facilities. Several layers of mathematical foundations are developed, including lenses to model variables and state spaces as algebraic objects, alphabetised predicates and relations to model programs, including algebraic and axiomatic semantics, proof tools for Hoare logic and refinement calculus, and UTP theories to encode computational paradigms.

==> sec/prelim.tex <==
\noindent In this section we review some preliminary material, and highlight related work.

\subsection{Unifying Theories of Programming}
\label{sec:UTP}

Starting from Hehner's predicative programming~\cite{Hehner1984-PredicativeProgramming,Hehner1988}, Hoare and He developed the semantic techniques of Unifying Theories of Programming (UTP)~\cite{Hoare1994,Hoare&98,Cavalcanti&06}. They use Tarski's relational calculus~\cite{Tarski41} to define programming and modelling language theories. Their technique uses alphabetised binary relations to model programs as predicates~\cite{Hehner1984-PredicativeProgramming,Hehner1990}. These relations map an initial value of a variable such as $x$ to its later value, $x'$. These might be program variables or observations of the real world. For example, $clock : \nat$ is a variable that records the passage of time. It makes no sense to assign arbitrary values to $clock$, as this would model time travel. Healthiness conditions constrain observations using idempotent functions on predicates. For example, application of $\healthy{HT}(P) \defs (P \land clock \le clock')$ gives a predicate that forbids travelling backwards in time.

The choice of observational variables and healthiness conditions defines a UTP theory. This is a subset of the predicates of the relational calculus whose elements are the fixed points of the healthiness conditions. We use theories to capture the semantics of computational paradigms. A signature gives the syntax of each theory. We must show that each operator in the syntax is a closure over the theory: applying the operator to elements of the theory gives healthy results. An algebra then gives the relationship between elements of the theory. 

Hoare and He give theories of imperative  sequential and concurrent programs~\cite{Hoare&98}. Oliveira et al. combine these two paradigms in a mechanised theory~\cite{Oliveira&09}. Sherif et al. define real-time programs~\cite{Sherif2010}. Santos et al. define a theory of object orientation~\cite{SCS06}. Foster et al. define theories for hybrid systems combining discrete and continuous behaviour~\cite{Foster16b,Foster17b}. Bresciani defines a theory of probabilistic systems~\cite{Bresciani2012} and He et al. show how to define such a theory as an extension of a standard programming theory~\cite{HeMM2004}. Woodcock et al. formalise this theory~\cite{WoodcockCFMY2019}.

UTP theories are lattices of predicates ordered by the refinement relation: $S \refinedby P$. That is, program $P$ satisfies specification $S$. Most theories define this relation as universal inverse implication: everywhere, $P$ implies $S$. We prove such statements using Isabelle/UTP~\cite{Foster16a}.

\subsection{Isabelle/HOL}


Isabelle/HOL~\cite{Isabelle} is a proof assistant for Higher Order Logic (HOL). It consists of the Pure meta-logic, and the HOL object logic. Pure provides a term language, polymorphic type system, syntax translation framework for extensible parsing and pretty printing, and an inference engine. The jEdit-based IDE allows \LaTeX-like term rendering using Unicode. Isabelle theories consist of type declarations, definitions, and theorems proved by theorem composition. Theorems have the form of $\llbracket P_1; \cdots; P_n \rrbracket \Longrightarrow Q$, where $P_i$ is an assumption, and $Q$ is the conclusion. We prove things in Isabelle using tactics, which automate proof steps. The simplifier tactic, \textsf{simp}, rewrites terms using equational theorems $f(x_1 \cdots x_n) \equiv y$, where the right-hand side is smaller than the left-hand side. The \textsf{auto} tactic combines \textsf{simp} with deductive reasoning using introduction, elimination, and destruction rules. Isabelle also has the powerful \textsf{sledgehammer} proof method~\cite{Blanchette2011} which invokes external first-order automated theorem provers and SMT solvers on a proof goal, verifying their results internally using tactics like \textsf{simp} and \textsf{metis}, which is a first-order resolution prover. We construct proof tactics and strategies using the ML programming language.


HOL implements a functional programming language founded on an axiomatic set theory. This object logic gives us a principled approach to mechanised mathematics. We construct definitions and theorems by applying axioms in the proof kernel. HOL provides inductive datatypes, recursive functions, and records. It provides basic types, including sets ($\power A$), total functions ($A \to B$), numbers ($\nat$, $\num$, $\mathbb{R}$), and lists. These types can be parametric: $[nat]list$.\footnote{The square brackets are not used in Isabelle; we add them for readability.} Specialisation unifies two types if one is an instantiation of the type variables of the other. For example, $[nat]list$ specialises $[\alpha]list$, where $\alpha$ is a type parameter.

Types in Isabelle/HOL have non-empty carrier sets. The fundamental command for defining new types is the \ckey{typedef} command. This creates a parametric type based on a non-empty subset of an existing type. For example, $prime : \nat \to \bool$ is true if a given number is prime; defining the set $\{n : \nat | prime(n)\}$ requires that we exhibit at least one prime number. The $\ckey{datatype}$ command creates an algebraic data type with a finite number of constructors. The $\ckey{record}$ command creates a record type with several fields.

Isabelle supports the mechanisation of algebraic structures and specifications. Locales~\cite{Ballarin06} provide axiomatic specifications of an algebraic structure. They rely on abstract sort types, a collection of signature operators over the sorts, and axioms that constrain the behaviour of the operators. They provide theorems that follow from the axioms. 

For example, a semigroup structure requires a single sort $A$, a binary operator ($\cdot : A \to A \to A$), and an associativity axiom ($(x \cdot y)\cdot z = x \cdot (y \cdot z)$). We can instantiate locales with a concrete set of types and functions, if we can prove that the functions obey the axioms. For example, we can instantiate the semigroup locale with $[A]list$ and the list concatenation function ($xs \cat ys$), which is associative. Locales form hierarchies, with child locales adding further operators and axioms. 

Type classes restrict locales to a single type sort. They use Isabelle's polymorphic overloading to characterise the algebraic operators. This for instance allows us to overload $+$ with several definitions for different types.


\subsection{Mechanising UTP}
\label{sec:mech-utp}

Mechanising UTP requires a tool to support construction and verification of UTP theories. Nuka and Woodcock~\cite{Nuka2006-UTP}, Oliveira et al.~\cite{Oliveira07} and Feliachi et al.~\cite{Feliachi2010} embed UTP into an existing logic (HOL for the latter two). This allows them to harness existing proof automation. The exception is $U\!\cdot\!(TP)^2$ tool~\cite{Butterfield2010,Butterfield2012}. This is a bespoke proof assistant for UTP still in the early stages of development. 

A semantic embedding of UTP requires a model of alphabetised relations~\cite[Chapter~2]{Hoare&98}. To be acceptable, this must mimic the way people use UTP with pen-and-paper. To be useful, the model must give access to the automated proof facilities of the host logic.

In Hoare and He's book~\cite{Hoare&98}, an alphabetised relation is a pair $(\alpha P, P)$. The set $\alpha P$ contains variable declarations of the form $x : t$. The predicate $P$ containing no free variables other than those in $\alpha P$. As in the Z notation~\cite{Spivey89,WoodcockD1996}, we decorate a variable $x'$ to denote an output (or `after') variable. An input variable is undecorated. We partition the  alphabet into inputs and outputs: $\alpha P = \inalpha P \cup \outalpha P$.

Alphabets provide information used by programming operators to calculate the semantics of compositions. For example, in the sequential composition,  $P \relsemi Q$, we identify the output variables of $P$ with the input variables of $Q$.  Compatibility requires that $\outalpha P = \inalpha' Q$. We use alphabets in the concurrent composition $P \parallel Q$ to determine whether shared variables. Alphabets also determine how we observe programs in a theory: if a program is stable, if it has terminated, how many resources it holds, what the heap looks like.

Nuka and Woodcock created the earliest mechanisation of UTP~\cite{Nuka2006-UTP}. They develop a deep embedding of the alphabetised relational calculus in ProofPower-Z, a proof assistant built on HOL.\footnote{\url{www.lemma-one.com/ProofPower/doc/doc}.} They provide an abstract syntax tree for predicates, a semantic domain, and an interpretation function. Their semantic domain is $Pred \defs (\power \textit{Var}) \times (\power \textit{Binding})$. The first component is an alphabet. The second is a set of possible observations, a \textit{Binding}. They model this as a partial function from variables to values: $\textit{Binding} \defs (\textit{Var} \pfun \textit{Value})$. The set of observations is equal to a predicate over the observation space of type $\textit{Binding} \to \bool$.

UTP depends on a formalisation of alphabetised relations. This depends on a formalisation of free variables, a syntactic property of predicates. This requires an abstract syntax tree for predicates. Oliveira et al. point out that fixing an abstract syntax tree runs against an important doctrine in UTP~\cite{Oliveira07}. This is that UTP should have an extensible syntax to support the unification of heterogeneous semantics. 

Oliveira et al.'s mechanisation of UTP in ProofPower-Z omits the abstract syntax tree~\cite{Oliveira07}. Instead, they define semantic operators that are like $\textit{Pred}$~\cite{Nuka2006-UTP}. This results in a shallow embedding.  The absence of an abstract syntax tree means that there is no longer a concept of free variables. This presents problems in the side conditions of programming laws. Oliveira et al. solve this problem using `unrestriction'. This is a semantic idea: a predicate does not \emph{depend} on particular variables. We adopt this concept in Isabelle/UTP.


Oliveira et al.'s mechanisation omits an explicit formalisation of types~\cite{Oliveira07}. This leads to difficulties in alphabet declaration. This motivated Zeyda and Cavalcanti to extend that work by adding a type model and a typing relation~\cite{Zeyda2012}.  This has proved to be essential for mechanising UTP theories. Zeyda and Cavalcanti develop a hierarchy of theories from imperative programs through to reactive programs. This work lacks support for native type checking and proof automation. Formalising the typing relation means that it is necessary to prove typing side conditions. This hampers proof. 

Foster et al. tackle this problem by providing a `shallow layer' on the predicate model~\cite{Foster14}. This harnesses the Isabelle type system to discharge typing provisos. The work places an extra burden on the user: they must define their own \textit{Value} type. Proof is also hampered by the need to discharge alphabet provisos. For example, the composition $P \relsemi Q$ is well-formed if $\outalpha(P) = \inalpha(Q)$. We must prove this property, as it is not checked automatically.

Feliachi et al. take a different approach in their development of a UTP theorem prover in Isabelle/HOL~\cite{Feliachi2010,Feliachi2012}. Like Nuka and Woodcock~\cite{Nuka2006-UTP} and Oliveira et al.~\cite{Oliveira07}, they model predicates as sets of observations $\power \mathcal{S}$. This set is not \textit{Binding}, but any definable type in Isabelle/HOL. They use record types to encode observation spaces, where each field corresponds to a variable. This results in a great improvement in proof automation in their tool. They parametrise the predicate type by an observation space type $\alpha$. Their record type declarations double as alphabets. This means that the type checker is directly harnessed in checking alphabet provisos. The type $[\alpha]\textit{relation} \defs [\alpha \times \alpha]\textit{predicate}$, denotes a homogeneous relation whose alphabet is $\alpha$. Sequential composition has type $[\alpha]\textit{relation} \to [\alpha]\textit{relation} \to [\alpha]\textit{relation}$, and so this rejects relational compositions with incompatible alphabets.

They harness type inference to automatically assign a polymorphic alphabet type to a relation. Textbook UTP decorates the assignment operator $x :=_A v$ with an explicit alphabet $A$. We must provide this set to infer the alphabet. This annotation is often omitted for convenience by Hoare and He~\cite{Hoare&98}. But this is safe only when we can infer the alphabet unambiguously. By harnessing type inference, we can omit such explicit decorations. This results in relations that are well-formed by construction.

Besides overcoming the problems with alphabets and types, Feliachi et al. overcome the need for an explicitly formalised universe, \textit{Value}~\cite{Feliachi2010,Feliachi2012}. Other works need this~\cite{Nuka2006-UTP,Oliveira07,Zeyda2012,Foster14}. Since any type in HOL must have an \emph{a priori} fixed cardinality, it is impossible to construct a type universe into which we can inject any HOL type. This is not a problem for Feliachi et al., as their predicates are parametric~\cite{Feliachi2010,Feliachi2012}. An observation space type can make use of any HOL type for its variables. Zeyda and Cavalcanti also get round this problem~\cite{Zeyda16}. They have a distinguished type universe but at the expense of extending HOL with extra axioms.

In our development of Isabelle/UTP, we follow the direction taken by Feliachi et al.~\cite{Feliachi2010,Feliachi2012}. In particular, we use the type system for alphabet inference as this greatly improves automation. We adopt ideas from Oliveira et.~\cite{Oliveira07}, Zeyda and Cavalcanti ~\cite{Zeyda2012}, and Foster et al.~\cite{Foster14}. Most notably, we adopt unrestriction, because Feliachi et al.'s variable model does not permit us to form such properties of variables~\cite{Feliachi2010,Feliachi2012}. To understand this, we need to look more closely at how we should model observation spaces. These two mechanisation families represent two unique approaches to modelling observations. We look at these in the next section.

\subsection{Observation Space Modelling}

The principal difference between the UTP mechanisations described in the last section is their approach to modelling the observation space $\mathcal{S}$. Schirmer and Wenzel provide a general discussed on modelling state spaces~\cite{Schirmer2009}. 
They identify four common ways of mechanising the modelling of state: using (1) functions; (2) tuples, (3) records, and (4) abstract types. The first and third seem the most prevalent.


The first approach models state as a function $\textit{Var} \to \textit{Value}$, for suitable value and variable types. Nuka and Woodcock~\cite{Nuka2006-UTP}, Oliveira et al.~\cite{Oliveira07}, Foster et al.~\cite{Foster14}, Dongol et al,.~\cite{Dongol2015}, and Zeyda and cavalcanti~\cite{Zeyda16} all take this approach. It requires a deep model of variables and values. Concepts such as names and typing are first-class citizens. This provides an expressive model with few limitations on possible manipulations~\cite{Foster14}. Schirmer and Wenzel highlight two obstacles~\cite{Schirmer2009}. First, the machinery required for deep reasoning about program values is heavy and \emph{a priori} limits possible constructions. Second, explicit variable naming involves syntactic issues like substitution and $\alpha$-renaming. Zeyda and Cavalcanti mitigate the first issue by axiomatically introducing a value universe~\cite{Zeyda16}. But the complexities associated with the second issue remain. Once names and types are first-class citizens, it becomes necessary to replicate a large part of the underlying proof system meta-logic. This requires great effort and can hit proof efficiency. Even so, the approach seems necessary to model the dynamic creation of variables, as required, for example, in modelling memory heaps in separation logic~\cite{Calcagno2007,Dongol2015}.

The alternative approach uses records to model state; a technique often used by verification tools in Isabelle~\cite{Alkassar2008,Feliachi2010,Feliachi2012,Armstrong2015}. In particular, Feliachi et al. use this approach to create their semantic embedding of the UTP in Isabelle/HOL~\cite{Feliachi2010}. A record field represents a variable in this model. These can be abstractly represented using pairs of field-query and update functions, $f_i$ and $f_i\textit{-upd}$. We do not need to encode the set of variable names (\textit{Var}) in this approach. As Feliachi et al.~\cite{Feliachi2010,Feliachi2012} and Armstrong et al.~\cite{Armstrong2015} have shown, this approach greatly simplifies automation of program verification. This is in comparison with the former functional approach through directly harnessing, rather than replicating, the polymorphic type system and automated proof tactics. The expense is a loss of flexibility compared to the functional approach, particularly in the decomposition of state spaces. Implementations using records seldom provide general support for syntactic concepts like free variables and substitution.


Isabelle/UTP generalises both these models by abstractly characterising the behaviour of state and variables algebraically using lenses. It can achieve both a high level of proof automation like Feliachi et al.~\cite{Feliachi2010,Feliachi2012}, but also supports syntactic queries such as unrestriction and substitution. J.~Foster created lenses as an abstraction for bidirectional programming and solving the view-update problem~\cite{Foster09}. Lenses abstract different views of a state-space and allow their manipulation independently of the context. A lens consists of two functions: $\lget$ that extracts a view from a larger source, and $\lput$ that puts back an updated view. Fischer gives a detailed study of the algebraic lens laws for these functions~\cite{Fischer2015}. J.~Foster et al. also provide combinators for composing lenses~\cite{Foster07,Foster09}. The \emph{Boomerang} language uses lenses for transformations on textual data structures.\footnote{Boomerang home page: \url{http://www.seas.upenn.edu/~harmony/}}

Our lens approach relates to the Schirmer and Wenzel's state-space solution~\cite{Schirmer2009}, where they use Isabelle locales to characterise a state type abstractly and polymorphically. A difference though is their use of explicit names, where our lenses are nameless. A similar concept to lenses exists in Back's refinement calculus~\cite[Chapter~5]{Back1998}, which substantially pre-dates the work on lenses. Here, $\lget$ is \textsf{val}, the `access function', and $\lput$ is \textsf{set}, the `update function'. In spite of this, the three lens axioms are all present. A difference is that, unlike lenses, Back does not provide explicit models for the variable axioms~\cite{Back1998}.

\subsection{Embedding Logics}

There is a long tradition of embedding one logic in another. For example, it's well known that we can embed classical logic can into intuitionistic logic~\cite{vanDalen2001}. A simple embedding is a negative translation, based on Glivenko's theorem. This translation maps each classical formula $\phi$ into its double negation $\lnot \lnot \phi$. Glivenko's theorem states the following. If $\phi$ is a propositional formula, then $\phi$ is a classical tautology if and only if $\lnot \lnot \phi$ is an intuitionistic tautology. This translation has applications in the consistency of different formulations of arithmetic.

Mechanical theorem proving makes use of many logics: equational, first-order, higher-order, modal, temporal, linear, and dynamic. Providing an interactive proof development environment for all these logics is a huge challenge~\cite{HarperHP1993}. The system must handle syntax, binding operators, substitution, formulas, terms, and rules. It must represent, check, and construct formal proofs. This has led to the development of logical frameworks. These isolate the uniformities of wide classes of logics. The implementation of new logics share the existing proof infrastructure for the framework. The Edinburgh Logical Framework defines a presentation language for defining logical systems~\cite{HarperHP1993}. This implements a logic-independent proof development environment.

Melham shows how to define a recursive type in HOL to model CMOS circuits~\cite{Melham1988}. The constructors represent composition operators combining primitive components. This is an embedding of the language of circuit terms in higher-order logic. It models the structural aspects of the class of all CMOS circuit designs. The semantics of circuit terms is then described in two different ways. The first gives the switch model of transistor behaviour. The second gives the threshold switching model.

Boulton et al. build on Melham's work on hardware description languages (HDLs)~\cite{BoultonGGHHT1992}. In doing so, so they introduce what appears to be the first use in the literature of the terms `shallow embedding' and `deep embedding'. They distinguish two approaches to embedding HDLs in logic. The first is to represent the abstract syntax of HDL programs by terms. They then define within the logic semantic functions that assign meanings to the programs. The second is to define semantic operators in the logic. They then arrange that the user-interface parses input from HDL syntax directly to semantic structures. They call the former a deep embedding and the latter a shallow embedding.

Bowen and Gordon present a shallow embedding of Z in HOL~\cite{BowenG1995}. They give a motivating example involving a propositional language~\cite{BowenG1995}:
\[
  wff ::= \mathsf{True} | \mathsf{N}~wff | \mathsf{C}~wff~wff
\]
In a deep embedding, they represent $wff$s inside the host logic. Then they define a semantic function to interpret the language, again in the host logic:
\[
  \mathcal{M}(\mathsf{True}) = T \also%
  \mathcal{M}(\mathsf{N}~w) = \lnot \mathcal{M}(w) \also%
  \mathcal{M}(\mathsf{C}~w_1~w_2) = \mathcal{M}(w_1) \land \mathcal{M}(w_2)
\]
\newcommand{\parsesto}{\mathrel{\leadsto}}%
Their shallow embedding approach uses a parser to translate $wff$s into terms in the host logic. So, instead of having the object language constant $\mathcal{M}$ , we have a metalanguage procedure $Trans$. Let $\leadsto$ denote the parsing relation. Then the shallow embedding is:
\[
  Trans(\mathsf{True}) \parsesto ``T'' \also%
  Trans(\mathsf{N}~w) \parsesto ``\lnot'' \cat Trans(w) \also%
  Trans(\mathsf{C}~w_1~w_2) \parsesto Trans(w_1) \cat ``\land'' \cat Trans(w_2)
\]
They can prove theorems about our propositional language in a deep embedding. For example, they can prove that negation is an involution: $\forall w: wff @ w = \mathsf{N}\mathsf{N}w$. In a shallow embedding, the only theorems that they can prove are those actually in the host language. The negation-involution theorem is not expressible and so not provable.

As Bowen and Gordon note, deep and shallow embeddings are at opposite ends of a spectrum. Between them are hybrid embeddings with semantics both formalised in the host logic and programmed in the interface.

Gordon et al. also embed ACL2 in HOL~\cite{GordonHKR2006} and Gordon and Collavizza embed Hoare in HOL~\cite{GordonC2010}.

Von Wright has implemented the refinement calculus in HOL~\cite{Wright1994}. Back and von Wright have used this implementation to check most of the theorems presented in their book~\cite{ButlerGLRvW1997,LangbackaRW1995}.



==> sec/verify-machine.tex <==
In this section we draw together the collected results from sections~\ref{sec:lenses}, \ref{sec:isabelle-utp}, and
\ref{sec:utp-thy} to construct an automated verification tool for the graphical state machine notation, RoboChart, in
Isabelle/UTP. We begin by describing the RoboChart language in more detail, and then proceed to construct the tool in
Isabelle.

\subsection{RoboChart}

RoboChart~\cite{Miyazawa2017,Miyazawa2019-RoboChart} describes robotic systems in terms of a number of controllers that communicate using
shared channels. Each controller has a well defined interface, and its behaviour is described by one or more state
machines. A machine has local state variables and constants, and consists of nodes and transitions, with behaviour
specified using a formal action language~\cite{Oliveira&09}. Advanced features such as hierarchy, shared variables,
real-time constraints, and probability are supported.

A machine, \textsf{GasAnalysis}, is shown in Figure~\ref{fig:gasanalysis}; we use it as a running example. It models a
component of a chemical detector robot~\cite{Timmis2012} that searches for dangerous chemicals using its spectrometer
device, and drops flags at such locations. \textsf{GasAnalysis} is the component that decides how to respond to a sensor
reading. If gas is detected, then an analysis is performed to see whether the gas is above or below a given
threshold. If it is below, then the robot attempts to triangulate a position for the source location and turns toward
it, and if it is above, it stops.

\begin{figure}
  \vspace{-4ex}
  \begin{center}
    \includegraphics[width=.75\linewidth]{figures/GasAnalysis}
  \end{center}
  \vspace{-4.2ex}
  \caption{\textsf{GasAnalysis} state machine in RoboChart}
  \label{fig:gasanalysis}
  \vspace{-3ex}
\end{figure}

The interface consists of four events. The event $gas$ is used to receive sensor readings, and $turn$ is used to
communicate a change of direction. The remaining events, $resume$ and $stop$ carry no data, and are used to communicate
that the robot should resume its searching activities, or stop. The state machine uses four state variables: $sts$ to
store the gas analysis status, $gs$ to store the present reading, $ins$ to store the reading intensity, and $anl$ to
store the angle the robot is pointing. It also has a constant $thr$ for the gas intensity threshold. RoboChart provides
basic types for variables and constants, including integers, real numbers, sets, and sequences (\textit{Seq(t)}). The
user can also define additional types, that can be records, enumerations, or entirely abstract. For example, the type
\textit{Status} is an enumerated type with constructors \textit{gasD} and \textit{noGas}.

The behaviour is described by 6 nodes, including an initial node (\textit{i}); a final node (\textit{F}); and four
states: \textit{NoGas}, \textit{Analysis}, \textit{GasDetected}, and \textit{Reading}. The transitions are decorated
with expressions of the form \textit{trigger}[\textit{condition}]/\textit{statement}. When the event \textit{trigger}
happens and the guard \textit{condition} is true, then \textit{statement} is executed, before transitioning to the next
state. All three parts can optionally be omitted. RoboChart also permits states to have entry, during, and exit
actions. In our example, both \textit{Analysis} and \textit{GasDetected} have entry actions.

Modelling with RoboChart is supported by the Eclipse-based
RoboTool\footnote{\url{https://www.cs.york.ac.uk/circus/RoboCalc/robotool/}}, from which Figure~\ref{fig:gasanalysis}
has been captured. RoboTool automates verification via model checking using FDR4, and its extension to incorporate the
verification approach presented here is ongoing work.

\subsection{Static Semantics}

In this section we formalise the static semantics of state machines in Isabelle/HOL, which describes the variables,
transitions, and nodes. The meta-model, presented below, is based on the untimed subset of RoboChart, but note that our
use of UTP ensures that our work is extensible to more advanced semantic
domains~\cite{Sherif2010,Bresciani2012,Foster17b}. For now we omit constructs concerned with interfaces, operations,
shared variables, during actions, and hierarchy, and focus on basic machines.

\begin{definition}[State Machine Meta-Model]
  \noindent

  \begin{center}
  \begin{tabular}{rl}
    StMach ::=& \ckey{statemachine}~ID~ \\
                   & ~~ \ckey{vars} NameDecl* \ckey{events} NameDecl*  \ckey{states} NodeDecl*\\ 
                   & ~~  \ckey{initial} ID \ckey{finals} ID* \ckey{transitions} TransDecl* \\[1ex]
    NameDecl      ::=& ID [\ckey{:} Type] \\[1ex]
    NodeDecl     ::=& ID \ckey{entry} Action \ckey{exit} Action \\[1ex]
    TransDecl    ::=& ID \ckey{from} ID \ckey{to} ID \ckey{trigger} Event \ckey{condition} Expr \ckey{action} Action
  \end{tabular}
\end{center}
\end{definition}

\noindent A state machine is composed of an identifier, variable declarations, event declarations, state declarations,
an initial state identifier, final state identifiers, and transition declarations. Each variable and event consists of a
name and a type. A state declaration consists of an identifier, entry action, and exit action. A transition declaration
consists of an identifier, two state identifiers for the source and target nodes, a trigger event, a condition, and a
body action. Transitions with no trigger are denoted by null event ($\nulle$) which can be hidden later.

We implement the meta-model syntax using Isabelle's parser, and implement record types $[s, e]\textit{Node}$ and
$[s, e]\textit{Transition}$, that correspond to the \textit{NodeDecl} and \textit{TransDecl} syntactic categories. They
are both parametric over the state-space $s$ and event types $e$. \textit{Node} has fields $nname : \textit{string}$,
$nentry : [s, e]\Action$, and $nexit : [s,e]\Action$, that contain the name, entry action, and exit
action. \textit{Transition} has fields $src : \textit{string}$, $tgt : \textit{string}$, $trig : [s, e]\Action$,
$cond : [s]\upred$, and $act : [s, e]\Action$, that contain the source and target, the trigger, the condition, and the
body. Triggers are denoted by actions because they may correspond to multiple possible events. We create a record type
to represent a state machine.

\begin{definition}[State Machine Record Type]
  $$\ckey{record}~[s, e]\textit{StMach} ~~=~~ \begin{array}{l}
     \begin{array}{ll} init : ID & finals : [ID]list \\[.5ex]
        nodes : [[s, e]Node]list \quad& transs : [[s, e]Transition]list
      \end{array}
    \end{array}$$
\end{definition}

\noindent It declares four fields for the initial state identifier (\textit{init}), final states identifiers
(\textit{finals}), nodes definitions (\textit{nodes}), and transition definitions (\textit{transs}), and constitutes the
static semantics. Since this corresponds to the meta-model, and to ensure a direct correspondence with the parser, we do
not directly use sets and maps, but only lists in our structure. We will later derive views onto the data structure
above, that build on well-formedness constraints.

Below, we show how syntactic machines are translated to Isabelle definitions.

\begin{definition}[Static Semantics Translation]
$$
  \begin{array}{l}
    \ckey{statemachine}~s \\[1ex]
    ~ \ckey{vars}~x_1 : \tau^v_1 ~\cdots~ x_i : \tau^v_i \\[1ex]
    ~ \ckey{events}~e_1 : \tau^e_1 ~\cdots e_j~ : \tau^e_j \\[1ex]
    ~ \ckey{states}~s_1 \cdots s_k ~ \ckey{initial}~ini \\[1ex]
    ~ \ckey{finals}~f_1 \cdots f_m \\[1ex]
    ~ \ckey{transitions}~t_1 \cdots t_n
  \end{array}
  ~~~\Longrightarrow~~~~~ \begin{array}{l}
  \ckey{alphabet}~\textit{s-alpha} = x_1 : \tau^v_1 ~\cdots~ x_i : \tau^v_i \\[1ex]
  \ckey{datatype}~\textit{s-ev} = \nulle | e_1~t^e_1 | \cdots | e_j~t^e_j \\[1ex]
  \ckey{definition}~ machine : [\text{s-alpha}, \text{s-ev}]\text{StMach} \\[1ex]
  \ckey{where}~machine = \begin{array}{l}
                           \llparenthesis init = ini, \\ 
                              ~finals = [f_1 \cdots f_m], \\
                              ~states = [s_1 \cdots s_k], \\
                              ~transs = [t_1 \cdots t_n] \rrparenthesis
                          \end{array} \\ \\[-2.5ex]
  \ckey{definition}~ semantics = \msem{machine}
\end{array}
$$
\end{definition}
\noindent For each machine, a new observation space $\ssdef{\textit{s-alpha}}{x_1 : \tau^v_1 ~\cdots~ x_i : \tau^v_i}$
is created, and lenses for each field of the form $\tau^v_i \lto \textit{s-alpha}$. For the events, an algebraic
datatype \textit{s-ev} is created with constructors corresponding to each of them. We create a distinguished event
$\nulle$ that will be used in transitions that not specify an explicit trigger event, which ensures that every
transition has at least one visible event. This in turn ensures that the resulting reactive program is productive, as
required by Theorem~\ref{thm:iterintro}. The overall machine static semantics is then contained in \textit{machine}. We
also define \textit{semantics} that contains the dynamic semantics in terms of the semantic function $\msem{\cdot}$ that
we describe in \S\ref{sec:dynsem}.

Elements of the meta-model are potentially not well-formed, for example specifying an initial state without a
corresponding state declaration, and therefore it is necessary to formalise well-formedness. RoboTool enforces a number
of well-formedness constraints~\cite{Miyazawa2018RoboChart,Miyazawa2019-RoboChart}, and we here formalise the subset needed to ensure the
dynamic semantics given in \S\ref{sec:dynsem} can be generated. We need some derived functions for this, and so we
define $nnames \defs set(map~nname~(nodes))$, which calculates the set of node names, and $fnames$, which calculates the
set of final node names. We can now specify our well-formedness constraints.
\begin{definition} \label{def:wfsm} A state machine is well-formed if it satisfies these constraints:
  \begin{enumerate}
    \item \textnormal{Each node identifier is distinct:} $distinct(map~nname~(nodes))$
    \item \textnormal{The initial identifier is defined:} $init \in nnames$
    \item \textnormal{The initial identifier is not final:} $init \notin fnames$
    \item \textnormal{Every transition's source node is defined and non-final:} \\ $\forall t \in transs @ src(t) \in nnames \setminus fnames$
    \item \textnormal{Every transition's target node is defined:} $\forall t \in transs @ tgt(t) \in nnames$
  \end{enumerate}
\end{definition}
\noindent We have implemented these constraints in Isabelle/HOL, along with a proof tactic called \textit{check-machine}
that discharges them automatically when a generated static semantics is well-formed, and ensures that crucial theorems
are available to the dynamic semantics. In practice, any machine accepted by RoboTool is well-formed, and so this tactic
simply provides a proof of that fact to Isabelle/HOL.

In a well-formed machine every node has a unique identifier. Therefore, using Definition~\ref{def:wfsm}, we construct
two finite partial functions, $\nmap : ID \ffun [s, e]\textit{Node}$ and
$\tmap : ID \ffun [s, e]\textit{Transition}~list$, that obtain the node definition and list of transitions associated
with a particular node identifier, respectively, whose domains are both equal to $\textit{nnames}$. We also define
$\textit{ninit} \defs \nmap~\textit{init}$, to be the definition of the initial node, and \textit{inters} to be the set
of nodes that are not final. Using well-formedness we can prove the following theorems.
\begin{theorem}[Well-formedness Properties] $ $

  \begin{enumerate}
    \item \textnormal{All nodes are identified:} $\forall n \in set(nodes) @ \nmap~(nname(n)) = n$
    \item \textnormal{The initial node is defined:} $ninit \in set(nodes)$
    \item \textnormal{The name of the initial node is correct:} $nname(ninit) = init$
  \end{enumerate}
\end{theorem}
\noindent These theorems allow us to extract the unique node for each identifier, and in particular for the initial
node. Thus, Isabelle/HOL can parse a state machine definition, construct a static semantics for it, and ensure that this
semantics is both well-typed and well-formed. The resulting Isabelle command is illustrated in
Figure~\ref{fig:rcisabelle} that encodes the \textsf{GasAnalysis} state machine of Figure~\ref{fig:gasanalysis}.

\begin{figure}[t]
  \vspace{-2ex}
  \begin{center}
    \includegraphics[width=.75\textwidth]{figures/Isabelle-StateMachine}
  \end{center}
  \vspace{-4ex}

  \caption{State machine notation in Isabelle/UTP}
  \label{fig:rcisabelle}

  \vspace{-2ex}
\end{figure}

\subsection{Dynamic Semantics}
\label{sec:dynsem}

In this section we describe the behaviour of a state machine using the reactive program domain we mechanised in
\S\ref{sec:actions}. The RoboChart reference semantics~\cite{Miyazawa2018RoboChart,Miyazawa2019-RoboChart} represents a state machine as a
parallel composition of CSP processes that represent the individual variables and states. Variable access and state
orchestration are modelled by communications between them. Here, we capture a simpler sequentialised semantics using
guarded iteration, which eases verification. In particular, state variables have a direct semantics, and require no
communication. The relation between these two semantics could, in the future, be formalised by an automated refinement
strategy that reduces parallel to sequential composition~\cite{Oliveira&09}.

We first define the observation space $\ssdef{[s]rcst}{actv : ID, \ckey{r} : s}$, parametrised by the state space type
$s$, and consisting of lenses $actv : ID \lto [s]rcst$ and $\ckey{r} : s \lto [s]rcst$. The $actv$ lens records the
currently active state, and $\ckey{r}$ projects the state machine variable space. No action is permitted to refer to
$actv$, a constraint that we impose through a frame extension operator, which we now consider.

Frame extension, $\frext{a}{P} : [s_1, e]\ukey{action}$, for $a : s_2 \lto s_1$ and $P : [s_2, e]\ukey{action}$, extends
the state space of $P$ using lens $a$. It is similar to a frame in refinement calculus~\cite{Morgan92}, which prevents
modification of variables, but also uses the type system to statically prevent access to them. Lens $a$ identifies a
subregion $s_2$, which $P$ acts upon, of the larger observation space $s_1$. Intuitively, $s_2$ specifies the set of
state machine variables, and $s_2$ extends it with $actv$. $P$ can only modify variables within $s_2$, and others are
held constant. We prove laws for this operator, which are also used in calculating the semantics.

\begin{theorem}[Frame Extension Laws] \label{thm:frext} 
  $$\frext{a}{P\!\relsemi\!Q} =~ \frext{a}{P}\!\relsemi\!\frext{a}{Q} \quad \frext{a}{e?x} =~ e?(\lns{a}{x}) \quad \frext{a}{x := v} =~ \lns{a}{x} := v$$
\end{theorem}

\noindent Frame extension distributes through sequential composition. For operators like event receive and assignment,
the variable is extended by the lens $a$ using a lens composition $x \lcomp a$ (see Def.~\ref{def:lenscomp}), which we
denote using a namespace-style operator ($\lns{a}{x}$). Specifically, it manipulates the region characterised by $x$
within the region of $a$.

We now describe the dynamic semantics of a state diagram using three functions.

\begin{definition}[Dynamic Semantics]
  \begin{align*}
    \msem{M} \defs~~& \left(\begin{array}{l}actv := init_M \relsemi \\ \doiter{N\!\in\!set(inters_M)}{actv = nname(N)}{\nsem{M}{N}} 
                      \end{array}\right)
    \\[.5ex]
    \nsem{M}{N} \defs~~ & 
        \frext{\ckey{r}}{nentry(N)} \relsemi \left(\Extchoice t\!\in\!\tmap_M(nname(N)) @ \trsem{M,N}{t}\right) \\[.5ex]
    \trsem{M,N}{t} \defs~~& \frext{\ckey{r}}{cond(t) \guard trig(t) \relsemi nexit(N) \relsemi action(t)} \relsemi actv := tgt(t)
  \end{align*}
\end{definition}

\noindent The function $\msem{\cdot} : [s, e]StMach \to [[s]rcst, e]\Action$ calculates the overall behavioural
semantics. It first sets $actv$ to the initial node identifier, and then enters a do iteration indexed by all non-final
nodes. If a final node is selected, then the iteration terminates. In each iteration, the node $N$ that is named by
$actv$ is selected, and the semantics for it is calculated using $\nsem{M}{N}$.

When in a node, the entry action is first executed using \textit{nentry}, and then an external choice is presented over
all transitions associated with $N$, which are calculated using $\tmap$. The entry and exit actions do not have $actv$
in their observation space, and therefore we apply frame extensions to them. The semantics of a transition,
$\trsem{M,N}{t}$, is guarded by the transition condition, and awaits the trigger event. Once this occurs, the exit
action of $N$ is executed, followed by the transition action, and finally $actv$ is updated with the target node
identifier.

The output of the semantics is an iterative program with one branch for every non-final state. To illustrate, we below
generate the denotational semantics for the \textsf{GasAnalysis} state machine given in Figure~\ref{fig:gasanalysis}.
\begin{example}[\textsf{GasAnalysis} Dynamic Semantics] \label{ex:gadynsem}

  $$\begin{array}{l}
      actv := InitState \relsemi \\[.2ex]
      \ckey{do} \\
      ~~~~\, actv = InitState \then \nulle \relsemi \lns{\ckey{r}}{gs} := \langle\rangle \relsemi \lns{\ckey{r}}{anl} := 0 \relsemi actv := NoGas \\[.2ex]
      ~~| actv = NoGas \then gas?\lns{\ckey{r}}{gs} \relsemi actv := Analysis \\[.2ex]
      ~~| actv = Analysis \then \\ 
          \quad~~ \lns{\ckey{r}}{sts} := analysis(\lns{\ckey{r}}{gs}) \relsemi 
          \left(\begin{array}{l}
             \lns{\ckey{r}}{sts} = noGas \guard \nulle \relsemi resume \relsemi actv := NoGas \\
            \extchoice \lns{\ckey{r}}{sts} = gasD \guard \nulle \relsemi actv := GasDetected 
          \end{array}\right) \\[1ex]
      ~~| actv = GasDetected \then \lns{\ckey{r}}{ins} := intensity(\lns{\ckey{r}}{gs}) \relsemi \\[.5ex]
      \qquad\qquad \left(\begin{array}{l}
               goreq(ins, thr) \guard \nulle \relsemi stop \relsemi actv := FinalState \\
               \extchoice (\neg goreq(ins, thr)) \guard 
                 \nulle \relsemi 
                       \begin{array}{l}
                         \lns{\ckey{r}}{anl} := location(\lns{\ckey{r}}{gs}) \relsemi \\
                         turn!(\lns{\ckey{r}}{anl}) \relsemi actv := Reading
                       \end{array}
                     \end{array}\right) \\[3ex]
      ~~| actv = Reading \then gas?\lns{\ckey{r}}{gs} \relsemi actv := Analysis \\[.5ex]
      \ckey{od}
    \end{array}$$
\end{example}
\noindent In order to yield a more concise definition, we have also applied the action equations, given in
Theorem~\ref{thm:frext} and \S\ref{sec:densemrea}, as simplification laws. In particular, the frame extensions have all
been expanded so that the state variables are explicitly qualified by lens $\ckey{r}$.

In order to verify such state machines, we need a specialised refinement introduction law. Using our well-formedness
theorem, we can specialise Theorem~\ref{thm:iterintro}.

\begin{theorem} \label{thm:stmref} The semantics of a state machine $M$ refines a reactive invariant specification $S$,
  that is $S \refinedby \msem{M}$, provided that the following conditions hold:
  \begin{enumerate}
    \item $M$ is well-formed according to Definition~\ref{def:wfsm};
    \item the initial node establishes the invariant --- $S \refinedby \nsem{M}{ninit_M}$;
    \item every non-final node preserves $S$ --- $\forall N \in inters_M @ S \refinedby S \relsemi (\nsem{M}{N})$.
  \end{enumerate}
\end{theorem}

\begin{proof}
  By application of Theorem~\ref{thm:iterintro}, and utilising trigger productivity.
\end{proof}


\noindent We now have all the infrastructure needed for verification of state machines, and in the next section we
describe our verification strategy and tool.

\subsection{Verification Strategy}
\label{sec:machvstrat}

In this section we use the collected results presented in the previous sections to define a verification strategy for
state machines, and exemplify its use in verifying deadlock freedom. Our approach utilises Theorem~\ref{thm:stmref} and
the contractual refinement tactic, \textsf{rdes-refine}~\cite{Foster17c}, which can be used to automatically show that a
reactive program $P$ satisfies (refines) a reactive contract: $\rc{S_1}{S_2}{S_3} \refinedby P$. We use this form to
prove that every state of a state machine satisfies a given invariant. The overall workflow for description and
verification of a state machine is given by the following steps:

\begin{enumerate}
  \item parse, type check, and compile the state machine definition;
  \item check well-formedness (Definition~\ref{def:wfsm}) using the \textit{check-machine} tactic;
  \item calculate denotational semantics, resulting in a reactive program;
  \item perform algebraic simplification and symbolic evaluation (Theorem~\ref{thm:ncsplaws});
  \item apply Theorem~\ref{thm:stmref} to produce sequential refinement proof obligations;
  \item apply \textsf{rdes-refine} to each goal, which may result in residual proof obligations;
  \item attempt to discharge each remaining proof obligation using \textsf{sledgehammer}~\cite{Blanchette2011}.
\end{enumerate}

This is effectively an elaborated version of the workflow followed by the \textsf{rel-auto} tactic we described in
\S\ref{sec:autoproof}. Diagrammatic editors, like RoboTool, can be integrated with the proof tool by implementing a
serialiser for the underlying meta-model. The workflow can be completely automated since there is no need to enter
manual proofs, and the final proof obligations are discharged by automated theorem provers. If proof fails, Isabelle/HOL
has the \textsf{nitpick}~\cite{Blanchette2011} counterexample generator that can be used for debugging. This means that
the workflow can be hidden behind a graphical tool.

We can use the verification procedure to check deadlock freedom of a state machine using the reactive contract
$\textit{\textsf{dlockf}} \defs \textstyle\rc{\true}{\exists e @ e \notin \refu}{\true}$, an invariant specification
which states that in all quiescent observations, there is always an event that is not being refused. In other words, at
least one event is always enabled; this is the meaning of deadlock freedom. We can use this contract to check the
\textsf{GasAnalysis} state machine. For a sequential machine, deadlock freedom means that it is not possible to enter a
state and then make no further progress. Such a situation can occur if the outgoing transitions can all be disabled
simultaneously if, for example, their guards do not cover all possibilities.

\begin{figure}[t]
  \vspace{-2ex}
  
  \begin{center}
    \includegraphics[width=\textwidth]{figures/Isabelle-Proof}
  \end{center}
  \vspace{-3.5ex}

  \caption{Selection of deadlock freedom proof obligations in Isabelle/UTP}
  \label{fig:rcproofs}

  \vspace{-3.5ex}
\end{figure}

The result of applying the verification procedure up to step 5 is shown in Figure~\ref{fig:rcproofs}. At this stage, the
semantics for each node has been generated, and deadlock freedom refinement conjectures need to be proved. Isabelle
generates 6 subgoals, 3 of which are shown, since it is necessary to demonstrate that the invariant is satisfied by the
initial state and each non-final state. The first goal corresponds to the initial state, where no event occurs and the
variables $gs$ and $anl$, along with $actv$, are all assigned. The second goal corresponds to the \textsf{Analysis}
state. The state body has been further simplified from the form shown in Figure~\ref{ex:gadynsem}, since symbolic
evaluation has pushed the entry action through the transition external choice, and into the two guards. This is also the
case for the third goal, which corresponds to the more complex \textsf{GasDetected} state.

The penultimate step applies the \textsf{rdes-refine} tactic to each of the 6 goals. This produces 3 subgoals for each
goal, a total of 18 first-order proof obligations, and invokes the relational calculus tactic \textsf{rel-auto} on each
of them. The majority are discharged automatically, but in this case three HOL predicate subgoals remain. One of them
relates to the \textsf{Analysis} state, and requires that the constructors $noGas$ and $gasD$ of $Status$ are the only
cases for $sts$. If there was a third case, there would be a deadlock as the outgoing transition guards don't cover
this.

Finally, we execute \textsf{sledgehammer} on each of the three goals, which provides proofs and so completes the
deadlock freedom check. Thus, we have engineered a fully automated deadlock freedom prover for state machines.


